Pseudo-Deterministic Construction of Irreducible Polynomials over Finite Fields

We present a polynomial-time pseudo-deterministic algorithm for constructing irreducible polynomial of degree $d$ over finite field $\mathbb{F}_q$. A pseudo-deterministic algorithm is allowed to use randomness, but with high probability it must output a canonical irreducible polynomial. Our construction runs in time $\tilde{O}(d^4 \log^4{q})$. Our construction extends Shoup's deterministic algorithm (FOCS 1988) for the same problem, which runs in time $\tilde{O}(d^4 p^{\frac{1}{2}} \log^4{q})$ (where $p$ is the characteristic of the field $\mathbb{F}_q$). Shoup had shown a reduction from constructing irreducible polynomials to factoring polynomials over finite fields. We show that by using a fast randomized factoring algorithm, the above reduction yields an efficient pseudo-deterministic algorithm for constructing irreducible polynomials over finite fields.

==> common_macros.tex <==
% Built over http://jeffe.cs.illinois.edu/pubs/tex/jeffe.sty

\RequirePackage{latexsym,amssymb}
%\RequirePackage[fleqn]{amsmath}

\hyphenation{co-or-din-ate co-or-din-ates half-plane half-space stereo-iso-mers
stereo-iso-mer Round-table homol-ogous homol-ogy}

% ----------------------------------------------------------------------
%  Common abbreviations and words with accents
% ----------------------------------------------------------------------

% ---- LATIN ----
\newcommand{\etal}{\emph{et~al.}}			% and others
\newcommand{\vitae}{vit\ae{}}
\newcommand{\apriori}{\emph{a~priori}}
\newcommand{\aposteriori}{\emph{a~posteriori}}

% ---- FRENCH ----
\newcommand{\naive}{na\"{\i}ve}
\newcommand{\Naive}{Na\"{\i}ve}
\newcommand{\naively}{na\"{\i}vely}	% Okay, I know, this isn't French.
\newcommand{\Naively}{Na\"{\i}vely}
\newcommand{\cafe}{caf\'e}

% ---- GERMAN ----
\newcommand{\fur}{f\"ur}
\newcommand{\Universitat}{Universit\"at}
\newcommand{\Saarbrucken}{Saar\-br\"ucken}	% Bypass TeX hyphenation
\newcommand{\Zurich}{Z\"urich}

% ---- PORTUGESE (Hi Jorge!) ----
\newcommand{\Computacao}{Computa\c{c}\~ao}

% ---- PROPER NAMES (because I'm lazy) ----
\newcommand{\Benes}{Bene\v{s}}		% ...network
\newcommand{\Bezier}{B\'ezier}		% ...spline/curve/surface
\newcommand{\bezout}{b\'{e}zout}
\newcommand{\Bezout}{B\'{e}zout}
\newcommand{\Bjorner}{Bj\"orner}
\newcommand{\Bochis}{Bochi\c{s}}		% Daciana
\newcommand{\Boruvka}{Bor\.uvka}		% ...'s MST algorithm
\newcommand{\Bragger}{Br\"agger}
\newcommand{\Bronnimann}{Br\"onnimann}   \newcommand{\Herve}{Herv\'e}
\newcommand{\Bruckner}{Br\"uckner}
\newcommand{\Caratheodory}{Carath\'eodory}	% Constantin
\newcommand{\Chvatal}{Chv\'atal}         \newcommand{\Vasek}{Va\v{s}ek}
				\newcommand{\Joao}{Jo\~ao}	% Compa
\newcommand{\Cortes}{Cort\'es}		% Carmen
\newcommand{\Dujmovic}{Dujmovi\'c}	% Vida
				\newcommand{\Fredo}{Fr\'edo}	% Durand
\newcommand{\Erdos}{Erd\H{o}s}           
\newcommand{\Frechet}{Fr\'echet}
\newcommand{\Furedi}{F\"uredi}           \newcommand{\Zoltan}{Zolt\'an}
\newcommand{\Gauss}{Gau{\ss}}
\newcommand{\Godel}{G\"{o}del}
\newcommand{\Grobner}{Gr\"obner}		% ... basis
\newcommand{\grobner}{gr\"obner}		% ... basis
\newcommand{\Grunbaum}{Gr\"unbaum}	% Branko
\newcommand{\Hanoi}{Hano\"\i}		% Tower of...
\newcommand{\Hastad}{H{\aa}stad}
\newcommand{\Hrubes}{Hrube{\v{s}}}       % Pavel
\newcommand{\Jarnik}{Jarn\a'{\i}k}	% ...'s (`Prim's') MST algorithm
\newcommand{\Komlos}{Koml\'os}
\newcommand{\Kovari}{K\"ov\'ari}
\newcommand{\Lovasz}{Lov\'asz}           \newcommand{\Laszlo}{L\'aszl\'o}
\newcommand{\Matousek}{Matou\v{s}ek}     \newcommand{\Jiri}{Ji\v{r}\'\i}
\newcommand{\Mnev}{Mn\"ev}
\newcommand{\Mobius}{M\"obius}		% ... strip/transformation/function
\newcommand{\Mucke}{M\"ucke}		% Ernst
\newcommand{\ODunliang}{\'O'D\'unliang}
\newcommand{\Oleinik}{Ole\u{\i}nik}
                                \newcommand{\Janos}{J\'anos}     % Pach
\newcommand{\Palasti}{Pal\'asti}
				\newcommand{\Belen}{Bel\'en}	% Palop
\newcommand{\Petrovskii}{Petrovski\u{\i}}
\newcommand{\Pinar}{P\i nar}		% Ali
\newcommand{\Plucker}{Pl\"ucker}		% ... coordinates
\newcommand{\Poincare}{Poincar\'e}	% ... duality/halfplane
                                \newcommand{\Gunter}{G\"unter}   % Rote, Ziegler
\newcommand{\Sacristan}{Sacrist\'an}	% Vera
\newcommand{\Saskin}{\v{S}a\v{s}kin}
\newcommand{\Schomer}{Sch\"omer}
\newcommand{\Schonhardt}{Sch\"onhardt}	% ... polyhedron
\newcommand{\Schonhage}{Sch\"onhage}
\newcommand{\Sos}{S\'os}
\newcommand{\Stackel}{St\"ackel}		% Paul
\newcommand{\Szekely}{Sz\'ekely}
\newcommand{\Szemeredi}{Szemer\'edi}
\newcommand{\Toth}{T\'{o}th}		% Geza
\newcommand{\Turan}{Tur\'an}
\newcommand{\Ungor}{\"Ung\"or}		% Alper
\newcommand{\Voronoi}{Vorono\"i}		% ... diagram [for francophile pedants only]


% ---- Math structures -----

\newcommand{\Real}{\mathbb{R}}
\newcommand{\Proj}{\mathbb{P}}
\newcommand{\Hyper}{\mathbb{H}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Rational}{\mathbb{Q}}
\newcommand{\Field}{\mathbb{F}}
\newcommand{\Prob}{\mathbb{P}}

\newcommand{\N}{\Natural}
\newcommand{\Q}{\Rational}
\newcommand{\R}{\Real}
\newcommand{\Z}{\Integer}
\newcommand{\F}{\Field}
\newcommand{\Fp}{\Field_p}
\newcommand{\Fq}{\Field_q}
\newcommand{\K}{\mathbb{K}}

% ---- OPERATORS (requires amsmath) ----
\newcommand{\aff}{\operatorname{aff}}		
\newcommand{\area}{\operatorname{area}}
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\Aut}{\operatorname{Aut}}		% Automorphism group
\newcommand{\conv}{\operatorname{conv}}	
\newcommand{\E}{\operatornamewithlimits{\mathbb{E}}}			% Expectation: $\E[X]$ (like \Pr)
\newcommand{\Hom}{\operatorname{Hom}}		% Homomorphism group
\newcommand{\id}{\operatorname{id}}		% identity
\newcommand{\im}{\operatorname{im}}		% image
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\rel}{\operatorname{rel\,}}	% relative (interior, boundary, etc.)
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\vol}{\operatorname{vol}}		% volume

% ---- DELIMITER PAIRS ----
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\inparen}[1]{\left( #1 \right)}
\newcommand{\insquare}[1]{\left[ #1 \right]}
\newcommand{\inbrace}[1]{\left\{ #1 \right\}}
\newcommand{\inangle}[1]{\left\langle #1 \right\rangle}
\newcommand{\pfrac}[2]{\inparen{\frac{#1}{#2}}} % just something I use so often

% ----- Some math symbols -----
\newcommand{\union}{\cup}
\newcommand{\Union}{\mathop{\bigcup}}
\newcommand{\intersection}{\cap}
\newcommand{\Intersection}{\mathop{\bigcap}}
\newcommand{\setdef}[2]{\inbrace{ #1 \ : \ #2}}      % E.g: \setdef{x}{f(x) = 0}
\newcommand{\innerproduct}[2]{\inangle{#1,#2}}
\newcommand{\?}{\stackrel{?}{=}}

% DegreeOfExtension{L, K} = [L: K]
\newcommand{\DegreeOfExtension}[2]{[#1 \vcentcolon #2]}

% for Hasse Derivative
\newcommand{\dbar}{d\hspace*{-0.08em}\bar{}\hspace*{0.1em}}


==> lazy_macros.tex <==
\RequirePackage{xfrac}
% Complexity classes
% \renewcommand{\P}{\mathsf{P}}
% \makeatletter
% \@latex@warning{Note: redefining \backslash P }
% \makeatother

\newcommand{\NP}{\mathsf{NP}}
\newcommand{\coNP}{\mathsf{coNP}}

% \renewcommand{\L}{\mathsf{L}}
% \makeatletter
% \@latex@warning{Note: redefining \backslash L }
% \makeatother

\newcommand{\NL}{\mathsf{NL}}
\newcommand{\coNL}{\mathsf{coNL}}
\newcommand{\FL}{\mathsf{FL}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\NPSPACE}{\mathsf{NPSPACE}}
\newcommand{\coNPSPACE}{\mathsf{coNPSPACE}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\coNEXP}{\mathsf{coNEXP}}
\newcommand{\sharpP}{\mathsf{\#P}}
\newcommand{\numberP}{\sharpP}
\newcommand{\Ppoly}{\sfrac{\P}{\poly}}
\newcommand{\PH}{\mathsf{PH}}
\newcommand{\AM}{\mathsf{AM}}
\newcommand{\MA}{\mathsf{MA}}


\newcommand{\DTIME}{\operatorname{\mathsf{DTIME}}}
\newcommand{\NTIME}{\operatorname{\mathsf{NTIME}}}
\newcommand{\coNTIME}{\operatorname{\mathsf{coNTIME}}}
\newcommand{\DSPACE}{\operatorname{\mathsf{DSPACE}}}
\newcommand{\NSPACE}{\operatorname{\mathsf{NSPACE}}}
\newcommand{\ASPACE}{\operatorname{\mathsf{ASPACE}}}
\newcommand{\ATIME}{\operatorname{\mathsf{ATIME}}}
\newcommand{\TISP}{\operatorname{\mathsf{TISP}}}
\newcommand{\DTS}{\operatorname{\mathsf{DTS}}}
\newcommand{\SigmaTIME}[1]{\operatorname{\mathsf{\Sigma_{#1}-TIME}}}
\newcommand{\PiTIME}[1]{\operatorname{\mathsf{\Pi_{#1}-TIME}}}
\newcommand{\SIZE}{\operatorname{\mathsf{SIZE}}}
\newcommand{\RP}{\operatorname{\mathsf{RP}}}
\newcommand{\coRP}{\operatorname{\mathsf{coRP}}}
\newcommand{\BPP}{\operatorname{\mathsf{BPP}}}
\newcommand{\ZPP}{\operatorname{\mathsf{ZPP}}}
\newcommand{\NC}{\operatorname{\mathsf{NC}}}
\newcommand{\AC}{\operatorname{\mathsf{AC}}}
\newcommand{\IP}{\operatorname{\mathsf{IP}}}
\newcommand{\PromiseP}{\operatorname{\mathsf{PromiseP}}}
\newcommand{\PromiseNP}{\operatorname{\mathsf{PromiseNP}}}
\newcommand{\PromiseBPP}{\operatorname{\mathsf{PromiseBPP}}}


%%% Common problems studied.

\newcommand{\CircuitSAT}{\operatorname{Circuit-SAT}}
\newcommand{\CNFSat}{\operatorname{CNF-Sat}}
\newcommand{\SAT}{\operatorname{SAT}}
\newcommand{\ThreeCNFSAT}{\operatorname{3-CNF-Sat}}
\newcommand{\ThreeCol}{\operatorname{3-Col}}
\newcommand{\IndSet}{\operatorname{Ind-Set}}
\newcommand{\IntProgram}{\operatorname{Int-Program}}
\newcommand{\Taut}{\operatorname{TAUT}}
\newcommand{\Clique}{\operatorname{Clique}}
\newcommand{\DirPath}{\operatorname{Dir-Path}}
\newcommand{\UndirPath}{\operatorname{Undir-Path}}
\newcommand{\DirSTConn}{\operatorname{Dir-ST-Conn}}
\newcommand{\DirSTUnconn}{\operatorname{Dir-ST-Unconn}}
\newcommand{\TQBF}{\operatorname{TQBF}}
\newcommand{\GraphNonIso}{\operatorname{Graph-non-Iso}}
\newcommand{\Perm}{\operatorname{Permanent}}
\newcommand{\SharpSAT}{\operatorname{\#SAT}}

\newcommand{\RPnote}[1]{\textcolor{red}{\guillemotleft RP: #1 \guillemotright}}
\newcommand{\SRnote}[1]{\textcolor{blue}{\guillemotleft SR: #1 \guillemotright}}
\newcommand{\MRnote}[1]{\textcolor{Purple}{\guillemotleft MR: #1 \guillemotright}}

